In Search of Projectively Equivariant Networks

Equivariance of linear neural network layers is well studied. In this work, we relax the equivariance condition to only be true in a projective sense. We propose a way to construct a projectively equivariant neural network through building a standard equivariant network where the linear group representations acting on each intermediate feature space are "multiplicatively modified lifts" of projective group representations. By theoretically studying the relation of projectively and linearly equivariant linear layers, we show that our approach is the most general possible when building a network out of linear layers. The theory is showcased in two simple experiments.

==> tables/max_tnet_table.tex <==
\begin{tabular}{r|rrrr|rrrr}
\toprule
%%%% From python script
& \multicolumn{4}{c}{ Test time rotation 0°} & \multicolumn{4}{c}{ Test time rotation 15°} \\
     AUC @ & 5° & 10° & 15° & 20° & 5° & 10° & 15° & 20° \\
\midrule
    {RANSAC} & -/ 8.5 & -/13.8 & -/18.4 & -/22.3 & -/ 8.5 & -/13.9 & -/18.5 & -/22.4 \\
    {GraT-Net2-\,\!-} &  2.5/40.3 &  6.4/50.1 & 10.5/56.3 & 14.4/60.7 &  2.5/40.5 &  6.0/50.3 & 10.1/56.8 & 14.2/61.3 \\
    {GraT-Net3-\,\!-} &  2.1/38.0 &  6.0/47.3 &  9.9/53.4 & 13.7/57.8 &  2.2/38.0 &  6.0/47.4 &  9.9/53.7 & 13.7/58.1 \\
    {GraT-Net2} & 25.9/51.0 & 39.8/61.0 & 49.0/67.3 & 55.8/71.6 & 16.2/47.7 & 27.6/58.4 & 36.4/64.7 & 43.2/69.2 \\
    {GraT-Net3} & 26.0/49.8 & 39.1/60.7 & 47.9/66.9 & 54.6/71.0 & 15.3/46.4 & 25.6/57.3 & 33.8/64.1 & 40.3/68.5 \\
    {ET-Net2} & 49.2/56.5 & 62.5/66.9 & 70.1/72.9 & 75.0/76.9 & 35.0/53.5 & 49.9/64.0 & 59.1/70.1 & 65.2/74.2 \\
    {ET-Net3} & 50.4/57.7 & 63.4/67.8 & 70.9/73.6 & 75.5/77.3 & 35.3/53.7 & 50.2/64.5 & 59.4/70.8 & 65.4/74.9 \\
    {T-Net (retrained)} & 48.2/55.3 & 61.9/65.7 & 69.1/71.7 & 73.8/75.6 & 35.4/52.8 & 49.4/63.1 & 58.1/69.3 & 63.9/73.2 \\
    {T-Net} (paper) & 52.3/56.1 & - & - & 75.8/75.5 & - & - & - & - \\
    %%%%
\bottomrule
\end{tabular}

==> tables/robust_res_fig.tex <==

%   \centering
%    \scriptsize
%    \begin{minipage}{.6\textwidth}
%    \begin{tabular}{r| lllll}
%    \toprule 
%        3 layers & Equiv. &  $0^\circ$ aug. & $15^\circ$ aug. &   $30^\circ$ aug. &  $45^\circ$ aug. \\
        
%        \midrule
%     $0^\circ$ data &  8.16e-02  &  {\bf 4.15e-02}  &  4.74e-02  &  5.08e-02  &  1.17e+00 \\
%$15^\circ$ data &  8.76e-02  &  6.73e-02  &  5.96e-02  &  {\bf 4.84e-02}  &  1.17e+00 \\
%$30^\circ$ data &  8.88e-02  &  1.42e-01  &  1.15e-01  &  {\bf 6.33e-02}  &  1.18e+00 \\
%$45^\circ$ data &  {\bf 8.80e-02}  &  2.70e-01  &  2.23e-01  &  1.26e-01  &  1.20e+00 \\
%        \bottomrule
%    \end{tabular}\end{minipage}\begin{minipage}{.4\textwidth}
%    \includegraphics[width=.9\textwidth]{figures/result_augs_3_layers.png}
%    \end{minipage}
  
    
%    \begin{minipage}{.6\textwidth} \vfill 
%    \begin{tabular}{r| lllll}
%    \toprule 
%        4 layers & Equiv. &  $0^\circ$ aug. & $15^\circ$ aug. &   $30^\circ$ aug. &  $45^\circ$ aug. \\
%          $0^\circ$ data &  8.02e-02  &  4.82e-02  &  {\bf 3.99e-02}  &  5.22e-02  &  1.21e+00 \\
%$15^\circ$ data &  7.90e-02  &  7.36e-02  &  {\bf 5.33e-02}  &  5.61e-02  &  1.23e+00 \\
%$30^\circ$ data &  7.77e-02  &  1.52e-01  &  9.78e-02  &  {\bf 7.26e-02}  &  1.22e+00 \\
%$45^\circ$ data &  {\bf 7.86e-02}  &  2.67e-01  &  2.04e-01  &  1.29e-01  &  1.23e+00 
%\\
%        \bottomrule
%    \end{tabular}
%   \end{minipage}\begin{minipage}{.4\textwidth}
%    \includegraphics[width=.9\textwidth]{figures/result_augs_4_layers.png}
%    \end{minipage}
    
%   \begin{minipage}{.6\textwidth}
%    \begin{tabular}{r| lllll}
%    \toprule 
%        5 layers & Equiv. &  $0^\circ$ aug. & $15^\circ$ aug. &   $30^\circ$ aug. &  $45^\circ$ aug. \\
        
%        \midrule
%     $0^\circ$ data &  6.66e-02  &  {\bf 4.63e-02}  &  5.54e-02  &  4.88e-02  &  1.19e+00 \\
%$15^\circ$ data &  6.72e-02  &  6.99e-02  &  6.77e-02  &  {\bf 5.39e-02}  &  1.20e+00 \\
%$30^\circ$ data &  {\bf 6.76e-02}  &  1.34e-01  &  1.05e-01  &  7.22e-02  &  1.22e+00 \\
%$45^\circ$ data &  {\bf 6.95e-02}  &  2.38e-01  &  1.95e-01  &  1.30e-01  &  1.21e+00 \\
%        \bottomrule
%    \end{tabular}
%    \end{minipage}\begin{minipage}{.4\textwidth}\includegraphics[width=.9\textwidth]{figures/result_augs_5_layers.png} \end{minipage}
    
    \scriptsize
   
    \begin{tabular}{r| l @{\hspace{1.2\tabcolsep}} l | l @{\hspace{1.2\tabcolsep}} l | l @{\hspace{1.2\tabcolsep}} l | l @{\hspace{1.2\tabcolsep}} l | l @{\hspace{1.2\tabcolsep}} l}
    \toprule 
        3 layers & \multicolumn{2}{c}{Equiv.} &  \multicolumn{2}{c}{ $0^\circ$ aug.} & \multicolumn{2}{c}{$15^\circ$ aug.} &   \multicolumn{2}{c}{$30^\circ$ aug.} &  \multicolumn{2}{c}{$45^\circ$ aug.} \\
         & mean & $\sigma$ & mean & $\sigma$ & mean & $\sigma$ & mean & $\sigma$ & mean & $\sigma$\\
        \midrule
    $0^\circ$ data &  8.16e-02 & {\bf 6.40e-03}  &  {\bf 4.15e-02} & 6.74e-03  &  4.74e-02 & 1.06e-02  &  5.08e-02 & 1.83e-02  &  1.17e+00 & 1.60e-01 \\
$15^\circ$ data &  8.76e-02 & 9.16e-03  &  6.73e-02 & {\bf 7.47e-03}  &  5.96e-02 & 8.22e-03  &  {\bf 4.84e-02} & 1.50e-02  &  1.17e+00 & 1.68e-01 \\
$30^\circ$ data &  8.88e-02 & {\bf 9.96e-03}  &  1.42e-01 & 1.21e-02  &  1.15e-01 & 1.41e-02  & {\bf  6.33e-02} & 1.88e-02  &  1.18e+00 & 1.49e-01 \\
$45^\circ$ data &  {\bf 8.80e-02} & {\bf 1.06e-02}  &  2.70e-01 & 1.34e-02  &  2.23e-01 & 1.76e-02  &  1.26e-01 & 3.07e-02  &  1.20e+00 & 1.30e-01 \\
        \bottomrule
    \end{tabular}

    \begin{tabular}{r| l @{\hspace{1.2\tabcolsep}} l | l @{\hspace{1.2\tabcolsep}} l| l @{\hspace{1.2\tabcolsep}} l | l @{\hspace{1.2\tabcolsep}} l | l @{\hspace{1.2\tabcolsep}} l}
    \toprule 
       4 layers & \multicolumn{2}{c}{Equiv.} &  \multicolumn{2}{c}{ $0^\circ$ aug.} & \multicolumn{2}{c}{$15^\circ$ aug.} &   \multicolumn{2}{c}{$30^\circ$ aug.} &  \multicolumn{2}{c}{$45^\circ$ aug.} \\
         & mean & $\sigma$ & mean & $\sigma$ & mean & $\sigma$ & mean & $\sigma$ & mean & $\sigma$\\
        
        \midrule
    $0^\circ$ data &  8.02e-02 & 1.58e-02  &  4.82e-02 & 7.97e-03  &  {\bf 3.99e-02} & {\bf 1.55e-02}  &  5.22e-02 & 2.33e-02  &  1.21e+00 & 1.53e-01 \\
$15^\circ$ data &  7.90e-02 & {\bf 1.03e-02}  &  7.36e-02 & 1.37e-02  &  {\bf 5.33e-02} & 1.73e-02  &  5.61e-02 & 2.16e-02  &  1.23e+00 & 1.48e-01 \\
$30^\circ$ data &  7.77e-02 & {\bf 1.60e-02}  &  1.52e-01 & 2.81e-02  &  9.78e-02 & 2.46e-02  &  {\bf 7.26e-02} & 2.92e-02  &  1.22e+00 & 1.45e-01 \\
$45^\circ$ data &  {\bf 7.86e-02} & {\bf 1.64e-02}  &  2.67e-01 & 2.21e-02  &  2.04e-01 & 3.10e-02  &  1.29e-01 & 3.44e-02  &  1.23e+00 & 1.36e-01 \\
        \bottomrule
    \end{tabular}
    
    \begin{tabular}{r| l @{\hspace{1.2\tabcolsep}} l | l @{\hspace{1.2\tabcolsep}} l | l @{\hspace{1.2\tabcolsep}} l | l @{\hspace{1.2\tabcolsep}} l | l @{\hspace{1.2\tabcolsep}} l}
    \toprule 
       5 layers & \multicolumn{2}{c}{Equiv.} &  \multicolumn{2}{c}{ $0^\circ$ aug.} & \multicolumn{2}{c}{$15^\circ$ aug.} &   \multicolumn{2}{c}{$30^\circ$ aug.} &  \multicolumn{2}{c}{$45^\circ$ aug.} \\
         & mean & $\sigma$ & mean & $\sigma$ & mean & $\sigma$ & mean & $\sigma$ & mean & $\sigma$\\
        \midrule
    $0^\circ$ data &  6.66e-02 & {\bf 5.73e-03}  &  {\bf 4.63e-02} & 1.10e-02  &  5.54e-02 & 4.94e-02  &  4.88e-02 & 1.41e-02  &  1.19e+00 & 1.82e-01 \\
$15^\circ$ data &  6.72e-02 & {\bf 7.36e-03}  &  6.99e-02 & 1.85e-02  &  6.77e-02 & 6.03e-02  & {\bf 5.39e-02} & 1.88e-02  &  1.20e+00 & 1.89e-01 \\
$30^\circ$ data &  {\bf 6.76e-02 } & {\bf 8.03e-03}  &  1.34e-01 & 1.36e-02  &  1.05e-01 & 5.00e-02  &  7.22e-02 & 2.77e-02  &  1.22e+00 & 1.81e-01 \\
$45^\circ$ data &  {\bf 6.95e-02} & {\bf 9.42e-03}  &  2.38e-01 & 1.40e-02  &  1.95e-01 & 4.45e-02  &  1.30e-01 & 2.51e-02  &  1.21e+00 & 1.66e-01 \\
        \bottomrule
    \end{tabular}
    
   

%\begin{figure}
%    \begin{subfigure}[b]{.33\linewidth}
%        \includegraphics[width=\linewidth]{figures/3_layers_equiv.png}
%        \caption{}
%    \end{subfigure}\begin{subfigure}[b]{.33\linewidth}
%        \includegraphics[width=\linewidth]{figures/4_layers_equiv.png}
%        \caption{}
%    \end{subfigure}\begin{subfigure}[b]{.33\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{figures/5_layers_equiv.png}
%        \caption{}
%    \end{subfigure}
%            \caption{Average loss on non-rotated data. The green lines correspond to equivariant models, the blue ones to augmented non-equivariant models, and the red lines to non-augmented, non-equivariant models. The solid lines are models whose initial node features include \texttt{local svd}s, wereas the dotted lines correspond to those who do not. Best viewed in colour.}
%        \label{fig:nonrot}
%\end{figure}

%\begin{figure}
%    \begin{subfigure}[b]{.33\linewidth}
%        \includegraphics[width=\linewidth]{figures/3_layers_equiv_rot.png}
%        \caption{}
%    \end{subfigure}\begin{subfigure}[b]{.33\linewidth}
%        \includegraphics[width=\linewidth]{figures/4_layers_equiv_rot.png}
%        \caption{}
%    \end{subfigure}\begin{subfigure}[b]{.33\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{figures/5_layers_equiv_rot.png}
%        \caption{}
%    \end{subfigure}
%            \caption{Average loss on rotated data. The green lines correspond to equivariant models, the blue ones to augmented non-equivariant models, and the red lines to non-augmented, non-equivariant models. The solid lines are models whose initial node features include \texttt{local svd}s, wereas the dotted lines correspond to those who do not. Best viewed in colour.}
%        \label{fig:rot}
%\end{figure}



==> tables/svd_diff_table.tex <==
    \begin{tabular}{r| ll | ll | l}
         3 layers & \multicolumn{2}{c}{$0^\circ$ at test} & \multicolumn{2}{c}{$30^\circ$ at test}  & Rel. diff. \\
         & mean & $\sigma$ & mean & $\sigma$ & \\
         \midrule
         Equiv + svd &  7.84e-02 & 7.29e-03 &  7.73e-02 & 5.32e-03 &  {\bf +1.35\%} \\
Equiv &  8.28e-02 & 5.39e-03 &  8.29e-02 & 4.24e-03 &  -0.19 \% \\
$0^\circ$ + svd &  {\bf 4.15e-02} & 5.79e-03 &  1.13e-01 & 9.87e-03 &  -172 \% \\
$0^\circ$ &  4.80e-02 & 1.22e-02 &  1.27e-01 & 2.01e-02 &  -165\% \\
$30^\circ$ + svd &  4.16e-02 & 4.50e-03 &  {\bf 7.12e-02} & 3.09e-03 &  -71.2\% \\
$30^\circ$ &  5.14e-02 & 1.06e-02 &  8.40e-02 & 1.73e-02 &  -63.6\% \\
\bottomrule
    \end{tabular} \begin{tabular}{r| ll | ll | l}
     4 layers & \multicolumn{2}{c}{$0^\circ$ at test} & \multicolumn{2}{c}{$30^\circ$ at test}  & Rel. diff. \\
         & mean & $\sigma$ & mean & $\sigma$ & \\
         Equiv + svd &  6.49e-02 & 1.60e-03 &  6.48e-02 & 1.86e-03 &  +0.16\% \\
Equiv &  6.97e-02 & 2.89e-03 &  6.93e-02 & 2.63e-03 &  {\bf +0.58\%} \\
$0^\circ$  + svd&  3.47e-02 & 2.42e-03 &  1.05e-01 & 3.32e-03 &  -202\% \\
$0^\circ$  &  4.04e-02 & 8.36e-03 &  1.17e-01 & 1.87e-02 &  -190\% \\
$30^\circ$ + svd&  {\bf 3.43e-02} & 2.69e-03 &  {\bf 5.56e-02} & 3.27e-03 &  -61.7\% \\
$30^\circ$ &  4.13e-02 & 1.50e-02 &  6.40e-02 & 2.22e-02 &  -54.8\% \\
\bottomrule
    \end{tabular} \begin{tabular}{r| ll | ll | l}
         5 layers & \multicolumn{2}{c}{$0^\circ$ at test} & \multicolumn{2}{c}{$30^\circ$ at test}  & Rel. diff. \\
         & mean & $\sigma$ & mean & $\sigma$ & \\
         \midrule
        Equiv + svd &  5.94e-02 & 1.75e-03 &  5.93e-02 & 2.19e-03 &  0.25 \% \\
Equiv &  6.57e-02 & 2.72e-03 &  6.51e-02 & 2.75e-03 &  {\bf 0.93\%} \\
$0^\circ$ + svd &  4.20e-02 & 1.02e-02 &  1.12e-01 & 1.40e-02 &  -166\% \\
$0^\circ$ &  4.10e-02 & 1.17e-02 &  1.10e-01 & 1.24e-02 &  -168\% \\
$30^\circ$  + svd &  {\bf 2.77e-02} & 2.57e-03 &  {\bf 4.64e-02} & 3.49e-03 &  -67.8\% \\
$30^\circ$ &  3.63e-02 & 1.36e-02 &  5.69e-02 & 2.36e-02 &  -56.7\% \\
\bottomrule
    \end{tabular}
    
       %\begin{tabular}{r|ll | ll | ll | ll | ll | ll}
%    \toprule 
%    3 layers & \multicolumn{2}{c}{Equiv} & \multicolumn{2}{c}{Equiv, nosvd} & \multicolumn{2}{c}{$0^\circ$ aug.} & 
%    \multicolumn{2}{c}{$0^\circ$ aug. nosvd} & \multicolumn{2}{c}{$30^\circ$ aug.} & \multicolumn{2}{c}{$30^\circ$ aug. nosvd} \\  
%    \midrule
%    $0^\circ$ data &  7.84e-02 & 7.29e-03  &  8.28e-02 & 5.39e-03  &  4.15e-02 & 5.79e-03  &  4.80e-02 & 1.22e-02  &  4.16e-02 & 4.50e-03  &  5.14e-02 & 1.06e-02 \\
%$30^\circ$ data &  7.73e-02 & 5.32e-03 &  8.29e-02 %& 4.24e-03 &  1.13e-01 & 9.87e-03 &  1.27e-01 & 2.01e-02 &  7.12e-02 & 3.09e-03 &  8.40e-02 & 1.73e-02\\
%\midrule 
%Relative diff. &  {\bf + 1.17 \%}  &  0.22 \% &  -158\%  &  -175\%  & -68.4\%  &  -65.7\% \\
%    \end{tabular}
    


%    \begin{tabular}{r|llllll}
%    \toprule 
%    4 layers & Equiv & Equiv, nosvd & $0^\circ$ aug. & $0^\circ$ aug. nosvd & $30^\circ$ aug. & $30^\circ$ aug. nosvd \\  
%    \midrule
%   $0^\circ$ data &  6.46e-02  &  6.88e-02  &  3.49e-02  &  3.56e-02  &  {\bf 3.46e-02}  &  4.47e-02 \\
%$30^\circ$ data &  6.39e-02  &  6.85e-02  &  1.06e-01  &  1.07e-01  &  {\bf 5.57e-02}  &  6.93e-02 \\
%\midrule 
%Relative diff. &  {\bf + 1\%}  &  {-0.4 \%}  &  -205\%  &  -201\%  & -61\%  &  -55\% \\
%    \end{tabular}

%\
%    \begin{tabular}{r|llllll}
%    \toprule 
%   5 layers & Equiv & Equiv, nosvd & $0^\circ$ aug. & $0^\circ$ aug. nosvd & $30^\circ$ aug. & $30^\circ$ aug. nosvd \\  
%    \midrule
%$0^\circ$ data &  6.00e-02  &  6.59e-02  &  4.70e-02  &  4.54e-02  &  {\bf 2.80e-02}  &  3.40e-02 \\
%$30^\circ$ data &  5.94e-02  &  6.58e-02  &  1.19e-01  &  1.14e-01  &  {\bf 4.60e-02}  &  5.21e-02 \\
%\midrule 
%diff &  {\bf +1.02\%}  &  +0.19\%  &  -153\%  &  -152\% &  -64.5\%  & -53.3\% \\
%    \end{tabular}

==> tables/tnet_table.tex <==
\begin{tabular}{r|rrrr|rrrr}
\toprule
%%%% From python script
& \multicolumn{4}{c}{ Test time rotation 0°} & \multicolumn{4}{c}{ Test time rotation 15°} \\
     AUC @ & 5° & 10° & 15° & 20° & 5° & 10° & 15° & 20° \\
\midrule
    {RANSAC} & -/ 8.5 & -/13.8 & -/18.4 & -/22.3 & -/ 8.5 & -/13.9 & -/18.5 & -/22.4 \\
    \textbf{GraT-Net2-\,\!-} &  2.5/40.3 &  6.4/50.1 & 10.5/56.3 & 14.4/60.7 &  2.5/40.5 &  6.0/50.3 & 10.1/56.8 & 14.2/61.3 \\
    \textbf{GraT-Net3-\,\!-} &  2.1/38.0 &  6.0/47.3 &  9.9/53.4 & 13.7/57.8 &  2.2/38.0 &  6.0/47.4 &  9.9/53.7 & 13.7/58.1 \\
    \textbf{GraT-Net2} & 25.9/51.0 & 39.8/61.0 & 49.0/67.3 & 55.8/71.6 & 16.2/47.7 & 27.6/58.4 & 36.4/64.7 & 43.2/69.2 \\
    \textbf{GraT-Net3} & 26.0/49.8 & 39.1/60.7 & 47.9/66.9 & 54.6/71.0 & 15.3/46.4 & 25.6/57.3 & 33.8/64.1 & 40.3/68.5 \\
    \textbf{ET-Net2} & 47.9/56.2 & 61.6/66.5 & 69.5/72.5 & 74.5/76.5 & 35.0/52.7 & 49.6/63.5 & 58.9/69.9 & 65.1/74.1 \\
    \textbf{ET-Net3} & 49.7/57.1 & 62.8/67.2 & 70.1/73.0 & 75.0/76.8 & 35.2/52.2 & 50.0/63.4 & 58.9/69.9 & 65.1/74.2 \\
    {T-Net (retrained)} & 47.9/55.1 & 61.5/65.1 & 69.1/71.1 & 73.8/75.0 & 34.2/52.8 & 48.8/63.1 & 57.6/69.2 & 63.6/73.1 \\
    {T-Net} (paper) & 52.3/56.1 & - & - & 75.8/75.5 & - & - & - & - \\
%%%%
\bottomrule
\end{tabular}
